Hierarchical multimodal transformers for Multi-Page DocVQA

Document Visual Question Answering (DocVQA) refers to the task of answering questions from document images. Existing work on DocVQA only considers single-page documents. However, in real scenarios documents are mostly composed of multiple pages that should be processed altogether. In this work we extend DocVQA to the multi-page scenario. For that, we first create a new dataset, MP-DocVQA, where questions are posed over multi-page documents instead of single pages. Second, we propose a new hierarchical method, Hi-VT5, based on the T5 architecture, that overcomes the limitations of current methods to process long multi-page documents. The proposed method is based on a hierarchical transformer architecture where the encoder summarizes the most relevant information of every page and then, the decoder takes this summarized information to generate the final answer. Through extensive experimentation, we demonstrate that our method is able, in a single stage, to answer the questions and provide the page that contains the relevant information to find the answer, which can be used as a kind of explainability measure.

==> previous_architecture_section.tex <==
\subsection{Architecture} \label{subsec:architecture}
\textbf{Encoder}: T5 encoder is composed of a stack of transformer layers, which in turn they are composed of self-attention transformers and feed-forward neural networks. In \methodName each page of the document is separately passed to the encoder along with the question in order to extract the relevant information conveyed in that page necessary to answer the given question. To do this, a number of learnable special \pageToken tokens are prepended to the input sequence of each page, which is composed by a special pretext string that specifies the task to perform, the question and the OCRed text enriched with spatial embeddings. These \pageToken tokens are inspired by the BERT \clsToken token, which is used to represent the whole sentence at the encoder's output. In our case, they will encode a global representation of each page, with the relevant information regarding the question. However, since there is much more information in a document page than in a sentence, instead of a single token we use a set of $N$ \pageToken tokens to encode this information. In addition, recent document understanding literature~\cite{xu2020layoutlm, xu2021layoutlmv2, powalski2021going} has proved the value of introducing 2D layout information. Therefore, following~\cite{biten2022latr} we combine the semantics and layout information by embedding the text token and their bounding box using a lookup table for continuous encoding of one-hot vector representations and summing up all the representations together. Finally, we also increase the input sequence size to 1024 tokens to ensure that all tokens of each page can fit into the model. Therefore, the encoder can process 1024 tokens for each page, which results in a total of 20048 tokens taking into account the 20 pages.


\textbf{Decoder}: The decoder is the original T5~\cite{raffel2020exploring} decoder with the difference of the input data. In \methodName the decoder's input consist of the concatenation of all contextualized \pageTokenC tokens of all pages in the document. Hence, the answer is generated from a holistic representation of the document with the most relevant information of each page.

\textbf{Retrieval module}: In parallel to the the answer generation in the decoder, the contextualized \pageTokenC tokens are concatenated and passed through a classification layer that outputs the index of the page where the answer is found.

\input{tables/methods_results}

\subsection{Training procedure} \label{subsec:training_procedure}

\textbf{Pre-training}: To improve the page representation encoded by the \pageToken tokens and provide the self-attention mechanism with the layout information, we perform a layout-aware pre-training task following~\cite{biten2022latr}. The pre-training task consists in layout-aware denoising where a span of tokens is masked while the position information keeps unchanged. Therefore, the model objective is to predict such masked tokens by using the semantic of the contextual tokens and the layout information. Nevertheless, in this case the model must predict the masked tokens from the compact representation of the \pageToken tokens, so that the encoder learns to represent the most relevant information to afterwards predict the original tokens. During pre-training, we use single page documents, and use cross-entropy loss to predict the original unmasked text tokens. 

\textbf{Training}: During training, an input sequence for each page is created consisting of $N$ \pageToken tokens, $M$ question tokens and the $O$ OCRed recognized text tokens of the corresponding page summed with the encoding of the layout features. Following the flow described in Section~\ref{subsec:architecture}, the contextualized \pageToken tokens of all pages are fed into the decoder to generate the answer and into the retrieval module to predict the answer page index. However, while \methodName is efficient by using most of the original T5 architecture and keeping its model size. The training of the \methodName architecture requires much more memory since each page is passed separately through the encoder and it is necessary to compute the gradients for each page. Consequently, this is similar to have a batch size $P$ times bigger in the encoder compared to the original T5 encoder. While this could be tackled by parallelizing into different GPUs the gradients corresponding to a set of encoded pages, we offer an alternative strategy using limited resources. To circumvent this problem, we train the model on shortened versions of the documents with only two pages: the page where the answer is found plus the previous or posterior page. Even though this drops the overall performance of the model, as we show in \cref{appendix:train_doc_pages}, training with only 2 pages is enough to learn the hierarchical representation of the model achieving results close to the ones using the whole document, while offers a good trade-off in terms of memory requirements. 

\textbf{Decoder and retrieval fine-tuning}: After the training phase, the decoder and the retrieval module have been trained with the shortened version of the documents and therefore, can face a problem when dealing with the full documents up to 20 pages long. For this reason, we perform a final fine-tuning with the complete documents containing all pages, following the same setup as in the training phase, but with the encoder weights frozen.

==> tables/ablation_results.tex <==
\begin{table}[ht]
\renewcommand*{\arraystretch}{1.3}
\vspace{-10pt}
\small
\captionsetup{width=.85\textwidth}
\centering
\begin{tabular}{lccccrr}
\toprule
\multirow{2}{*}{\textbf{Model}} & 
    \multirow{2}{*}{\textbf{Vf}}    &
    \textbf{Answ. Pg. Mod.} &
    \textbf{Pt} &
    \textbf{Ft} & 
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{ANLS}}} &
    \multicolumn{1}{c}{\textbf{Ans. Pg. Acc.}} \\
    
& & \textbf{features} & \textbf{module}    & \textbf{decoder}   &  \multicolumn{1}{c}{}                               & \multicolumn{1}{c}{\textbf{precision}} \\
\midrule
                                    & \xmark & \xmark & \cmark  & \xmark  & 0.5577  & 59.00     \\
                                    & \xmark & \cmark & \xmark  & \xmark  & 0.5849  & 0.00      \\
\multirow{-1.75}{*}{\methodName}    & \cmark & \cmark & \cmark  & \xmark  & 0.6263  & 55.74     \\
                                    & \xmark & \cmark & \cmark  & \cmark  & 0.5864  & 81.47     \\
\bottomrule
\end{tabular}
\vspace{-1.5mm}
\caption{\textbf{\methodName ablation studies}. We study the effect of embedding each page into different amount of \pageToken tokens, the effect of the visual features, the answer page prediction module, the pretraining and last % phase where the retrieval module and the decoder are fine-tuned.}
fine-tuning phases of the decoder and answer page prediction module.}
\label{tab:ablation_results}
\vspace{-10pt}
\end{table}



% 39.96 --> 46.32

==> tables/ablation_results_old.tex <==
\begin{table*}[ht]
\renewcommand*{\arraystretch}{1.3}
\vspace{-10pt}
\small
\captionsetup{width=.85\textwidth}
\centering
\begin{tabular}{lcccccrrr}
\toprule
\multirow{2}{*}{\textbf{Ablation}} & \textbf{\pageToken} & \multirow{2}{*}{\textbf{Pretrain} }& \textbf{DIT} & \textbf{Retrieval} & \textbf{Fine-tune} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Accuracy}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{ANLS}}} & \multicolumn{1}{c}{\textbf{Retrieval}} \\
                                & \textbf{Tokens}     &                                   & \textbf{features} & \textbf{module}    & \textbf{decoder}   & \multicolumn{1}{c}{}                                   & \multicolumn{1}{c}{}                               & \multicolumn{1}{c}{\textbf{precision}} \\
\midrule
                                        & 1     & \xmark & \cmark & \cmark    & \xmark    & 34.88     & 0.4999    & 57.80    \\
                                        & 2     & \xmark & \cmark & \cmark    & \xmark    & 36.41     & 0.5405    & 57.81    \\
\multirow{-0.5}{*}{\pageToken tokens}   & 5     & \xmark & \cmark & \cmark    & \xmark    & 37.78     & 0.5745    & 58.70    \\
                                        & 10    & \xmark & \cmark & \cmark    & \xmark    & 40.57     & 0.5987    & 59.40    \\
                                        & 25    & \xmark & \cmark & \cmark    & \xmark    & 40.21     & 0.5956    & 59.01    \\
                                        & 50    & \xmark & \cmark & \cmark    & \xmark    & 39.10     & 0.5891    & 59.69    \\
\hdashline
Visual features                         & 10    & \xmark & \xmark & \cmark    & \xmark    & 39.07     & 0.5577    & 59.00     \\
\hdashline 
Answer page prediction module           & 10    & \xmark & \cmark & \xmark    & \xmark    & 39.81     & 0.5849    & 0.00      \\
\hdashline
Pretrain                                & 10    & \cmark & \cmark & \cmark    & \xmark    & 42.86     & 0.6263    & 55.74     \\
\hdashline
Finetune decoder                        & 10    & \xmark & \cmark & \cmark    & \cmark    & 42.10     & 0.5864    & 81.47     \\
\hdashline
No ablation                             & 10    & \cmark & \cmark & \cmark    & \cmark    & 48.28     & 0.6201    & 79.23     \\
\bottomrule
\end{tabular}
\vspace{-1.5mm}
\caption{\textbf{\methodName ablation studies}. We study the effect of embedding each page into different amount of \pageToken tokens, the effect of the visual features, the answer page prediction module, the pretraining and last % phase where the retrieval module and the decoder are fine-tuned.}
fine-tuning phases of the decoder and answer page prediction module.}
\label{tab:ablation_results}
\vspace{-10pt}
\end{table*}



% 39.96 --> 46.32

==> tables/ablation_results_old2.tex <==
\begin{table*}[ht]
\renewcommand*{\arraystretch}{1.3}
\vspace{-10pt}
\small
\captionsetup{width=.85\textwidth}
\centering
\begin{tabular}{lccccrrr}
\toprule
\multirow{2}{*}{\textbf{Ablation}} & \textbf{\pageToken} & \multirow{2}{*}{\textbf{Pretrain}} & \textbf{Retrieval} & \textbf{Fine-tune} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Accuracy}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{ANLS}}} & \multicolumn{1}{c}{\textbf{Retrieval}} \\
                                & \textbf{Tokens}     &                                    & \textbf{module}    & \textbf{decoder}   & \multicolumn{1}{c}{}                                   & \multicolumn{1}{c}{}                               & \multicolumn{1}{c}{\textbf{precision}} \\
\midrule
                                        & 1     & \xmark     & \cmark    & \xmark    & 31.93     & 0.4861    & 61.23     \\
                                        & 2     & \xmark     & \cmark    & \xmark    & 33.42     & 0.5015    & 57.42     \\
\multirow{-0.5}{*}{\pageToken tokens}   & 5     & \xmark     & \cmark    & \xmark    & 36.88     & 0.5374    & 58.30     \\
                                        & 10    & \xmark     & \cmark    & \xmark    & 39.07     & 0.5577    & 59.00     \\
                                        & 25    & \xmark     & \cmark    & \xmark    & 38.98     & 0.5549    & 58.74     \\
                                        & 50    & \xmark     & \cmark    & \xmark    & 38.59     & 0.5532    & 60.69     \\
\hdashline 
Retrieval module                        & 10    & \xmark    & \xmark    & \xmark    & 38.36     & 0.5433    & 0.00         \\
\hdashline
Pretrain                                & 10    & \cmark    & \cmark    & \xmark    & 43.86     & 0.6063    & 53.74     \\
\hdashline
Finetune decoder                        & 10    & \xmark    & \cmark    & \cmark    & 42.10     & 0.5864    & 80.37     \\
\hdashline
No ablation                                    & 10    & \cmark    & \cmark    & \cmark    & 46.32     & 0.5999    & 78.22           \\
\bottomrule
\end{tabular}
\vspace{-1.5mm}
\caption{\textbf{\methodName ablation studies}. We study the effect of embedding each page into different amount of \pageToken tokens, the effect of the retrieval module, pretraining and the last % phase where the retrieval module and the decoder are fine-tuned.}
fine-tuning phase of the decoder and retrieval module.}
\label{tab:ablation_results}
\vspace{-10pt}
\end{table*}



% 39.96 --> 46.32

==> tables/datasets_old.tex <==
\begin{table*}[ht]
\small \centering
% \begin{tabular}{lcccSSS}
\begin{tabular}{lcccSSS}
\toprule
% \textbf{Dataset} & \textbf{Questions} & \textbf{Documents} & \textbf{Pages (Images)} & \textbf{Question Avg. Length} & \textbf{Answer Avg. Length} & \textbf{Avg. Document Words} \\
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Questions}} & \multirow{2}{*}{\textbf{Documents}} & \multirow{2}{*}{\textbf{Pages (Images)}} & \textbf{Question}    & \textbf{Answer}      & \textbf{Document Avg.} \\
                                  &                                     &                                     &                                          & \textbf{Avg. length} & \textbf{Avg. length} & \textbf{OCR Tokens}    \\
\midrule
SingleDocVQA~\cite{mathew2021docvqa}            & 50K  &   \hspace{9pt}6K   &   \hspace{5pt}12K     &   9.49    &   2.43      & 151.46    \\
% SingleDocVQA~\cite{mathew2021docvqa}            & 50K  &   \hspace{5pt}12K   &   \hspace{5pt}12K     &   9.49    &   2.43      & 151.46    \\
VisualMRC~\cite{tanaka2021visualmrc}            & 30K  &   \hspace{5pt}10K  &   \hspace{5pt}10K     &   10.55   &   9.55      & 182.75    \\
InfographicsVQA~\cite{mathew2022infographicvqa} & 30K  &   \hspace{3pt}5.4K &   \hspace{3pt}5.4K    &   11.54   &   1.60      & 217.89    \\
DuReaderVis~\cite{qi2022dureadervis}            & 15K  &   158K             &   158K                &   9.87       &   180.54    & 1968.21   \\
DocCVQA~\cite{tito2021document}                 & 20   &   \hspace{5pt}14K  &   \hspace{5pt}14K     &   14.00   &   12.75     & 509.06    \\
TAT-DQA~\cite{zhu2022towards}                   & 16K  &   \hspace{3pt}2.7K &   \hspace{10pt}3K     &   12.54   &   3.44      & 494.04    \\
MP-DocVQA (ours)                                & 46K  &   \hspace{10pt}6K  &   \hspace{5pt}60K     &   9.90    &   2.20      & 2026.59   \\
\bottomrule
\end{tabular}
\vspace{-2pt}
\caption{Comparison between \datasetName and main DocVQA datasets.}
\vspace{-10pt}
\label{tab:datasets_stats}
\end{table*}

==> tables/datasets_old2.tex <==
\begin{table*}[ht]
\small \centering
% \begin{tabular}{lcccSSS}
\begin{tabular}{lcccSSS}
\toprule
% \textbf{Dataset} & \textbf{Questions} & \textbf{Documents} & \textbf{Pages (Images)} & \textbf{Question Avg. Length} & \textbf{Answer Avg. Length} & \textbf{Avg. Document Words} \\
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Questions}} & \multirow{2}{*}{\textbf{Documents}} & \multirow{2}{*}{\textbf{Pages (Images)}} & \textbf{Question}    & \textbf{Answer}      & \textbf{Document Avg.} \\
                                  &                                     &                                     &                                          & \textbf{Avg. length} & \textbf{Avg. length} & \textbf{OCR Tokens}    \\
\midrule
SingleDocVQA~\cite{mathew2021docvqa}            & 50K  &   6K   &   12K &   9.49    &   2.43      & 151.46    \\
VisualMRC~\cite{tanaka2021visualmrc}            & 30K  &   10K  &   10K &   10.55   &   9.55      & 182.75    \\
InfographicsVQA~\cite{mathew2022infographicvqa} & 30K  &   5.4K &  5.4K &   11.54   &   1.60      & 217.89    \\
DocCVQA~\cite{tito2021document}                 & 20   &   14K  &   14K &   14.00   &   12.75     & 509.06    \\
DuReaderVis~\cite{qi2022dureadervis}            & 15K  &   158K &  158K &   9.87    &   180.54    & 1968.21   \\
MP-DocVQA (ours)                                & 46K  &   6K   &   60K &   9.90    &   2.20      & 2026.59   \\
\bottomrule
\end{tabular}
\vspace{-2pt}
\caption{Comparison between \datasetName and main DocVQA datasets.}
\vspace{-10pt}
\label{tab:datasets_stats}
\end{table*}

==> tables/method_hyperparameters_old.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr} \toprule
                      & \multicolumn{1}{c}{\textbf{BERT}} &
                      \multicolumn{1}{c}{\textbf{Longformer}} &
                      \multicolumn{1}{c}{\textbf{BigBird}} &
                      \multicolumn{1}{c}{\textbf{T5}} \\
\midrule
Model size            & large       & base      & base      & base      \\
Parameters            & 334M        & 148M      & 131M      & 223M      \\
Model initial weigths & 
\href{https://github.com/mineshmathew/DocVQA/tree/master/BERT_baseline}{SingleDocVQA} & \href{https://huggingface.co/valhalla/longformer-base-4096-finetuned-squadv1}{SQuADv1}  & \href{https://huggingface.co/google/bigbird-base-trivia-itc}{TrivaQA}   & \href{https://huggingface.co/t5-base}{C4}                          \\
Max Seq. Length       & 512         & 4096      & 4096      & 512       \\
%                     &             &           &           &           \\
batch size            & 32          & 8         & 8         & 32        \\
lr                    & 2e-5        & 1e-4      & 3e-5      & 2e-4      \\
optimizer             & AdamW       & AdamW     & AdamW     & AdamW     \\
scheduler             & linear      & linear    & linear    & linear    \\
warmup iterations     & 1000        & 1000      & 1000      & 1000      \\
training epochs       & 1           & 10        & 10        & 10        \\
\bottomrule
\end{tabular}}
\caption{Hyperparameters of baselines and proposed method used to train and evaluate on \datasetName}
\label{tab:training_parameters}
\end{table}

==> tables/methods_results_old.tex <==
\begin{table*}[ht]
\centering
\small
% \resizebox{0.95\textwidth}{!}{
\vspace{-10pt}

\begin{tabular}{lcccrccc}
% \begin{tabular}{lcccP{0.10\linewidth}ccc}
% \begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} lccllrrr}
\toprule
    & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{}  & \textbf{Max Seq.} & \textbf{Retrieval} &  &   & \textbf{Retrieval}    \\
    
\multirow{-2}{*}{\textbf{Model}} & \multicolumn{1}{l}{\multirow{-2}{*}{\textbf{Size}}} & \multicolumn{1}{l}{\multirow{-2}{*}{\textbf{Parameters}}} & \textbf{Length}        & \textbf{mode}      & \multirow{-2}{*}{\textbf{Accuracy}} & \multirow{-2}{*}{\textbf{ANLS}} & \textbf{Precision}                   \\

\midrule
                            &       &       &       & Oracle    & 39.77     & 0.5904    & 100.00    \\
BERT~\cite{devlin2018bert}  & Large & 334M  & 512   & Concat    & 27.41     & 0.4183    &  \hspace{5pt}51.61    \\
                            &       &       &       & Logits    & 34.78     & 0.5347    &  \hspace{5pt}71.24    \\
\hdashline
                                         &      &       &       & Oracle    & 52.48     & 0.6177    & 100.00    \\
\longformer~\cite{beltagy2020longformer} & Base & 148M  & 4096  & Concat    & 43.91     & 0.5285    &  \hspace{5pt}71.17    \\
                                         &      &       &       & Logits    & 45.87     & 0.5506    &  \hspace{5pt}70.37    \\
\hdashline
                                &       &       &       & Oracle    & 55.39     & 0.6454    & 100.00    \\
\bigbird~\cite{zaheer2020big}   & Base  & 131M  &  4096 & Concat    & 41.06     & 0.4928    & \hspace{5pt}51.78     \\
                                &       &       &       & Logits    & 49.57     & 0.5854    & \hspace{5pt}72.27     \\
\hdashline
                                &       &       &       & Oracle    & 59.00     & 0.6814    & 100.00    \\
T5~\cite{raffel2020exploring}   & Base  & 223M  & 512   & Concat    & 41.80     & 0.5047    & \hspace{20pt}-- \\
                                &       &       &       & Logits    & 32.68     & 0.4028    & \hspace{5pt}46.05    \\
 % LAyoutT5
%   & & & & Oracle & & & \\
%   & & & & Concat & & & \\
%   \multirow{-3}{*}{Layout T5} & \multirow{-3}{*}{Base} & \multirow{-3}{*}{223M} & \multirow{-3}{*}{512} & Logits & & & \\
\hdashline
                                    &       &       &       & Oracle    & 39.99     & 0.6397    & 100.00 \\
LayoutLMv2~\cite{xu2021layoutlmv2}  & Base  & 200M  & 561   & Concat    & 26.06     & 0.4075    & 51.94  \\ % 512 + 49 = 561
%                                   &       &       &       & Logits    & 32.93     & 0.5383    & 67.76  \\
                                    &       &       &       & Logits    & 32.93     & 0.5083    & 67.76  \\
\hdashline
                                        &       &       &       & Oracle    & 59.21     & 0.6729    & 100.00 \\
LayoutLMv3~\cite{huang2022layoutlmv3}   & Base  & 125M  & 708   & Concat    & 38.47     & 0.4538    & 51.94  \\  % 512 + 196 = 708 + 2? [CLS] + [SEP]
%                                       &       &       &       & Logits    & 51.70     & 0.6016    & 74.02  \\
                                        &       &       &       & Logits    & 42.70     & 0.5513    & 74.02  \\
\hdashline
 & & & & Oracle & 49.57 & 0.6252 & 100.00 \\
\multirow{-1}{*}{\methodName (Ours)} & \multirow{-1}{*}{Base} & \multirow{-1}{*}{226M} & \multirow{-1}{*}{20480} & \methodName Ret. Module & \multirow{-0.5}{*}{46.32} & \multirow{-0.5}{*}{0.5999} & \multirow{-0.5}{*}{\hspace{5pt}78.22} \\

\bottomrule
% \end{tabular*}
\end{tabular}
%}
\vspace{-1.5mm}
\captionsetup{width=.87\textwidth}
\caption{\textbf{Baselines and proposed method \methodName results on \datasetName dataset}. Baselines are evaluated on three different setups: oracle, concat and logits. The proposed method evaluated only on the oracle setup and using its hierarchical architecture with the retrieval module.}
\vspace{-3mm}

\label{tab:methods_results}
\end{table*}
